Adaptive normalization for IPW estimation

Inverse probability weighting (IPW) is a general tool in survey sampling and causal inference, used both in Horvitz-Thompson estimators, which normalize by the sample size, and H\'ajek/self-normalized estimators, which normalize by the sum of the inverse probability weights. In this work we study a family of IPW estimators, first proposed by Trotter and Tukey in the context of Monte Carlo problems, that are normalized by an affine combination of these two terms. We show how selecting an estimator from this family in a data-dependent way to minimize asymptotic variance leads to an iterative procedure that converges to an estimator with connections to regression control methods. We refer to this estimator as an adaptively normalized estimator. For mean estimation in survey sampling, this estimator has asymptotic variance that is never worse than the Horvitz--Thompson or H\'ajek estimators, and is smaller except in edge cases. Going further, we show that adaptive normalization can be used to propose improvements of the augmented IPW (AIPW) estimator, average treatment effect (ATE) estimators, and policy learning objectives. Appealingly, these proposals preserve both the asymptotic efficiency of AIPW and the regret bounds for policy learning with IPW objectives, and deliver consistent finite sample improvements in simulations for all three of mean estimation, ATE estimation, and policy learning.

==> contents/coverage.tex <==
%!TEX root = ../TukeyTrotterDraft.tex

\newpage
\section{Confidence intervals and coverage}

In this section we discuss the problem of constructing confidence intervals for $\hat{\mu}_{\AN}$. Since we have computed the asymptotic variance of $\hat{\mu}_{\AN}$ in Theorem~\ref{thm:mu-hat-fp-clt}, we can use a normal approximation to construct confidence intervals that are asymptotically valid. The coverage of these intervals in a simulation experiment is shown in Figure~\ref{fig:coverage}.


\begin{figure}[t]
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.5\linewidth]{figures/coverage.pdf}&\includegraphics[width=0.48\linewidth]{figures/fixed_population_coverage.pdf}
\end{tabular}
\caption{The coverage of a 95\% confidence interval for $\hat{\mu}_{\text{HT}}$, $\hat{\mu}_{\Hajek{}}$, and $\hat{\mu}_{\AN}$ based on the asymptotic variances in Theorems~\ref{thm:mu-hat-lambda-clt} ($\lambda=0,1$) and \ref{thm:mu-hat-fp-clt} in a superpopulation model (left) and a fixed population model (right). In the superpopulation model, at each trial, the $Y_k, p_k, I_k$ are all drawn anew, while in the fixed population model, the $Y_k, p_k$ are fixed and the $I_k$ are drawn anew at each trial. The target coverage is indicated with a dashed line. The coverage in the fixed population model is significantly better than the coverage in the superpopulation model, for reasons discussed in the main text.}
	\label{fig:coverage}
\end{figure}


Unfortunately, we see that in the superpopulation model, which is the model we have considered throughout, the coverage is quite poor. To better understand the reason for this behavior, consider the asymptotic variance of the \Hajek{} estimator, $\E\left[ \frac{1-p_k}{p_k}(Y_k-\mu)^2 \right]$. Crucially, $p\mapsto \frac{1-p}{p}$ is a decreasing function of $p\in[0,1]$, and so this expectation up-weights small values of $p_k$. But these are exactly the values we are least likely to observe, hence the difficulty in obtaining an accurate approximation of the asymptotic variance, and thus in obtaining confidence intervals with good coverage. In particular, we do not believe that these results are due to a failure of the normal approximation: the normal approximation should be very nearly exactly correct for values as large as $n=1000$, but estimating the parameters of the target normal approximation remains challenging. This is further evidenced by the fact that $\hat{\mu}_{\text{HT}}$, for which there is no approximation and the asymptotic variance is exactly correct, actually has slightly lower coverage than $\hat{\mu}_{\text{HT}}$. Rather, the challenge is in estimating $\E\left[ \frac{1-p_k}{p_k}Y_k^2 \right]$, which is slightly harder than estimating the asymptotic variance of $\hat{\mu}_{\Hajek}$ because $Y_k^2$ is typically larger than $(Y_k-\mu)^2$.

This point is further demonstrated by the significantly improved coverage of the same intervals in the fixed population simulation in the right panel of Figure~\ref{fig:coverage}. In this setting, the asymptotic variance of, for example, the \Hajek{} estimator is no longer $\E\left[ \frac{1-p_k}{p_k}(Y_k-\mu)^2 \right]$ but is rather $\lim \frac{1}{n}\sum_{k=1}^n \frac{1-p_k}{p_k}(Y_k-\overline{Y})^2$ where the limit is over a sequence of finite populations of increasing size and $\overline{Y}=\frac{1}{n}\sum_{k=1}^n Y_k$. The improved coverage is driven by the fact that now, only the small values of $p_k$ that are actually in the finite population, rather than all possible values of $p_k$, contribute to the variance, and so there is less unobserved variance negatively impacting the coverage.

To summarize, intervals constructed using our theory show sub-par coverage in simulation, but this is largely due to unobserved variance in the problem and the difficulty of estimating such variance, as evidenced by the comparison with the finite population setting, rather than a failure of our theory or of the normal approximation. 

